k-way Hypergraph Partitioning via n-Level Recursive Bisection

We develop a multilevel algorithm for hypergraph partitioning that contracts the vertices one at a time. Using several caching and lazy-evaluation techniques during coarsening and refinement, we reduce the running time by up to two-orders of magnitude compared to a naive $n$-level algorithm that would be adequate for ordinary graph partitioning. The overall performance is even better than the widely used hMetis hypergraph partitioner that uses a classical multilevel algorithm with few levels. Aided by a portfolio-based approach to initial partitioning and adaptive budgeting of imbalance within recursive bipartitioning, we achieve very high quality. We assembled a large benchmark set with 310 hypergraphs stemming from application areas such VLSI, SAT solving, social networks, and scientific computing. We achieve significantly smaller cuts than hMetis and PaToH, while being faster than hMetis. Considerably larger improvements are observed for some instance classes like social networks, for bipartitioning, and for partitions with an allowed imbalance of 10%. The algorithm presented in this work forms the basis of our hypergraph partitioning framework KaHyPar (Karlsruhe Hypergraph Partitioning).

==> plots/bipartitioning_evaluation.tex <==
\begin{figure}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering \includegraphics[width=.45\textwidth]{./plots/figure/manual-bipartition_eval-1} 

}

\end{knitrout}
\caption{Performance plots for all hypergraphs, $k=2$ and $\varepsilon = 0.03$. Note the cube root scale for both axes.}\label{fig:bipart_eval}
\end{figure}



==> plots/makros.tex <==
% open issues
%\marginparwidth5cm
\marginparpush2mm
\marginparsep1mm 
%\newcommand{\frage}[1]{\makebox[0cm]{$\bigotimes$}\marginpar{\tiny #1}}
\newcommand{\frage}[1]{{[\bf #1]}\marginpar{$\bigotimes$}}

\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\etal}{et al.\xspace}




==> plots/running_time_full_benchmark.tex <==
\begin{figure}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering \includegraphics[width=.45\textwidth]{./plots/figure/manual-running_time_fullbench-1} 

}
\end{knitrout}
\caption{Running time ratio plot for all benchmark instances and $\varepsilon=0.03$. The log-scaled y-axis shows the ratio between the running time of the corresponding algorithm and the running time of the fastest algorithm. For each algorithm, the ratios are sorted in increasing order.}\label{fig:running_time}
\end{figure}



==> plots/websocial_evaluation.tex <==
\begin{figure*}
\centering
\begin{knitrout}
\definecolor{shadecolor}{rgb}{0.969, 0.969, 0.969}\color{fgcolor}

{\centering 
\centering \includegraphics[width=.45\textwidth]{./plots/figure/manual-bipartition_eval-1} 
\includegraphics[width=.45\textwidth]{./plots/figure/manual-websocial_eval-1} 

}
\end{knitrout}
\caption{Performance plots for web-crawls and social networks\footnotemark~for $\varepsilon = 0.03$. Note the cube root scale for both axes.}\label{fig:websocial_eval}
\end{figure*}

